Consistent circuits for indefinite causal order

Over the past decade, a number of quantum processes have been proposed which are logically consistent, yet feature a cyclic causal structure. However, there is no general formal method to construct a process with an exotic causal structure in a way that ensures, and makes clear why, it is consistent. Here we provide such a method, given by an extended circuit formalism. This only requires directed graphs endowed with Boolean matrices, which encode basic constraints on operations. Our framework (a) defines a set of elementary rules for checking the validity of any such graph, (b) provides a way of constructing consistent processes as a circuit from valid graphs, and (c) yields an intuitive interpretation of the causal relations within a process and an explanation of why they do not lead to inconsistencies. We display how several standard examples of exotic processes, including ones that violate causal inequalities, are among the class of processes that can be generated in this way; we conjecture that this class in fact includes all unitarily extendible processes.

==> new_process.tex <==
\input{preamble}
\input{commands}


\begin{document}

\section{Building a new process}

In these notes, we present a genuinely new process, built using our framework.

\subsection{A presentation at the logical level}
As with Lugano, this process can be presented as a non-causal voting scheme, whose outcomes affect the agents' ordering, and are made partially accessible to them before they cast their vote. In Lugano, a majority vote determined which of 3 agents acts after the others; this could easily be generalised to build Lugano processes on $N > 3$ parties, working in a similar way, with a majority vote determining one winner among the $N$ participants, that acts after all the others. The process we present here goes further: it showcases a voting scheme in which \textit{two} parties might get elected into two different roles. The two elected parties then act one after the other, and after all losing parties. 

The voting scheme can be described as the election, by 5 parties, of a president and a chancellor among themselves, with the president acting after the chancellor. In this scheme, only the losing parties cast a vote;\footnote{We could, as was done in our reconstruction of the Lugano, yield the winning parties a dummy vote, while making sure that the rules imply that it would never affect the outcomes; this would be irrelevant to the process' basic behaviour.} each hands over a `president-chancellor' ticket, i.e.\ votes for two people, with the constraint that one cannot vote for the same person as chancellor and president, and cannot vote for oneself in either office. The vote's outcome is determined as follows:

\begin{itemize}
    \item a party gets elected as president if they receive $\geq 3$ presidential votes;
    \item a party gets elected as chancellor either if they receive 4 cancellarial votes, or if they receive 3 cancellarial votes and these 3 votes all agreed on their presidential vote as well.
\end{itemize}

Note that it is possible that either or both of the positions end up not getting filled. A party learns, before acting, whether they have been appointed as chancellor or president or have lost the vote. On top of this, the agents act on arbitrarily large message systems in an order determined by the outcomes: all losing parties act first (spacelike to one another), then the chancellor if there's one, then the president if there's one. A late party can receive arbitrarily large messages from all parties that acted earlier. This is summed up in the following graph.

\be \tikzfig{ProcessSummary} \ee

If we strip off the democratic metaphors for a moment, the concrete novelty in this process is that two parties -- and not just one as in the Lugano process or its straightforward $N$-parties generalisations -- can get promoted to act last, and furthermore that the process yields a non-trivial ordering between these parties as well.

\end{document}
